Cookbook: A framework for improving LLM generative abilities via programmatic data generating templates

Fine-tuning large language models (LLMs) on instruction datasets is a common way to improve their generative capabilities. However, instruction datasets can be expensive and time-consuming to manually curate, and while LLM-generated data is less labor-intensive, it may violate user privacy agreements or terms of service of LLM providers. Therefore, we seek a way of constructing instruction datasets with samples that are not generated by humans or LLMs but still improve LLM generative capabilities. In this work, we introduce Cookbook, a framework that programmatically generates training data consisting of simple patterns over random tokens, resulting in a scalable, cost-effective approach that avoids legal and privacy issues. First, Cookbook uses a template -- a data generating Python function -- to produce training data that encourages the model to learn an explicit pattern-based rule that corresponds to a desired task. We find that fine-tuning on Cookbook-generated data is able to improve performance on its corresponding task by up to 52.7 accuracy points. Second, since instruction datasets improve performance on multiple downstream tasks simultaneously, Cookbook algorithmically learns how to mix data from various templates to optimize performance on multiple tasks. On the standard multi-task GPT4ALL evaluation suite, Mistral-7B fine-tuned using a Cookbook-generated dataset attains the best accuracy on average compared to other 7B parameter instruction-tuned models and is the best performing model on 3 out of 8 tasks. Finally, we analyze when and why Cookbook improves performance and present a metric that allows us to verify that the improvement is largely explained by the model's generations adhering better to template rules.

==> tables/inst-ws-nostd.tex <==
\begin{table*}[h!]
\centering
\scriptsize
\begin{tabular}{l|cccccccc|c}
\hline
\textbf{Model} & \textbf{arc\_c} & \textbf{arc\_e} & \textbf{boolq} & \textbf{hellaswag} & \textbf{lambada} & \textbf{openbookqa} & \textbf{piqa} & \textbf{winogrande} & \textbf{average} \\
\hline
\llama & 46.25 & 74.58 & 77.74 & 75.99 & 73.92 & 44.20 & 79.11 & 69.14 & 67.61 \\
\textsc{\llama-chat} & 44.20 & 69.74 & 79.76 & 75.50 & 71.08 & 43.80 & 77.20 & 66.46 & 65.97 \\
\textsc{\llama-NH} & 49.74 & 76.09 & 80.00 & 77.72 & 72.99 & \textbf{46.40} & 79.76 & 70.01 & 69.09 \\
\mistral & 54.10 & 79.50 & 83.49 & 81.12 & 75.59 & 44.40 & 82.05 & 73.88 & 71.76 \\
\textsc{\mistral-cap} & 54.01 & 78.54 & 82.57 & 78.74 & 72.46 & 44.80 & 79.60 & 71.03 & 70.22 \\
\textsc{\mistral-orca} & 56.14 & 79.59 & 86.57 & 81.73 & 72.37 & 45.60 & \textbf{83.03} & 73.24 & 72.28 \\
\textsc{\mistral-OH} & \textbf{59.98} & 81.65 & \textbf{86.73} & \textbf{81.77} & 73.90 & 44.20 & 82.70 & 73.56 & 73.06 \\
\hline
\textsc{TEMPLATE-LLAMA} & 48.04 & 76.77 & 79.20 & 76.04 & 77.10 & 43.40 & 78.56 & 69.30 & 68.55 \\
\textbf{\textsc{TEMPLATE-MISTRAL}} & 59.39 & 82.79 & 86.15 & 81.17 & 78.36 & 43.80 & 82.37 & 73.56 & \textbf{73.45} \\
\textsc{\mistral-unif} & 58.70 & 82.66 & 79.97 & 81.09 & \textbf{78.46} & 43.60 & 81.77 & \textbf{75.06} & 72.66 \\
\textsc{\mistral-ws} & 57.76 & \textbf{83.21} & 85.23 & 80.99 & 78.23 & 44.00 & 82.32 & 74.27 & 73.25 \\
\end{tabular}
\caption{\textbf{Model performance on the GPT4ALL benchmark.} ``temp'' denotes our template tuned models, ``NH'' denotes NousHermes Dataset, ``cap'' is the Nous-Capybara models, ``OH'' is Open-Hermes, and ``orca'' is OpenOrca. Averaged across tasks, \mistral-temp is the best performing model.}
\label{tab:model_performance_nostd}
\end{table*}

==> tables/inst.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{l|cccccccc|c}
\hline
\textbf{Model} & \textbf{arc\_c} & \textbf{arc\_e} & \textbf{boolq} & \textbf{hellaswag} & \textbf{lambada} & \textbf{openbookqa} & \textbf{piqa} & \textbf{winogrande} & \textbf{avg} \\
\hline
mistral-OO & 55.38 \scriptsize{± 1.45} & 82.74 \scriptsize{± 0.78} & 86.57 \scriptsize{± 0.60} & 63.87 \scriptsize{± 0.48} & 72.37 \scriptsize{± 0.62} & 36.20 \scriptsize{± 2.15} & 81.18 \scriptsize{± 0.91} & 73.24 \scriptsize{± 1.24} & 68.94 \scriptsize{± 1.03} \\
llama2 & 43.43 \scriptsize{± 1.45} & 76.35 \scriptsize{± 0.87} & 77.74 \scriptsize{± 0.73} & 57.14 \scriptsize{± 0.49} & 73.92 \scriptsize{± 0.61} & 31.40 \scriptsize{± 2.08} & 78.07 \scriptsize{± 0.97} & 69.14 \scriptsize{± 1.30} & 63.40 \scriptsize{± 1.06} \\
mistral-Cap & 50.43 \scriptsize{± 1.46} & 78.96 \scriptsize{± 0.84} & 82.57 \scriptsize{± 0.66} & 60.77 \scriptsize{± 0.49} & 72.46 \scriptsize{± 0.62} & 33.00 \scriptsize{± 2.10} & 79.27 \scriptsize{± 0.95} & 71.03 \scriptsize{± 1.27} & 66.06 \scriptsize{± 1.05} \\
mistral-OH & 56.23 \scriptsize{± 1.45} & 83.33 \scriptsize{± 0.76} & 86.73 \scriptsize{± 0.59} & 63.15 \scriptsize{± 0.48} & 73.90 \scriptsize{± 0.61} & 34.80 \scriptsize{± 2.13} & 81.39 \scriptsize{± 0.91} & 73.56 \scriptsize{± 1.24} & 69.14 \scriptsize{± 1.02} \\
llama2-NH & 47.61 \scriptsize{± 1.46} & 79.46 \scriptsize{± 0.83} & 80.00 \scriptsize{± 0.70} & 59.35 \scriptsize{± 0.49} & 72.99 \scriptsize{± 0.62} & 36.60 \scriptsize{± 2.16} & 78.78 \scriptsize{± 0.95} & 70.01 \scriptsize{± 1.29} & 65.60 \scriptsize{± 1.06} \\
llama2-synth & 45.99 \scriptsize{± 1.46} & 77.44 \scriptsize{± 0.86} & 79.20 \scriptsize{± 0.71} & 57.32 \scriptsize{± 0.49} & 77.10 \scriptsize{± 0.59} & 33.80 \scriptsize{± 2.12} & 78.24 \scriptsize{± 0.96} & 69.30 \scriptsize{± 1.30} & 64.80 \scriptsize{± 1.06} \\
mistral-synth & 54.78 \scriptsize{± 1.45} & 83.29 \scriptsize{± 0.77} & 86.15 \scriptsize{± 0.60} & 61.40 \scriptsize{± 0.49} & 78.36 \scriptsize{± 0.57} & 32.60 \scriptsize{± 2.10} & 81.45 \scriptsize{± 0.91} & 73.56 \scriptsize{± 1.24} & 68.95 \scriptsize{± 1.02} \\
llama2-chat & 44.20 \scriptsize{± 1.45} & 73.86 \scriptsize{± 0.90} & 79.76 \scriptsize{± 0.70} & 57.79 \scriptsize{± 0.49} & 71.08 \scriptsize{± 0.63} & 33.20 \scriptsize{± 2.11} & 76.39 \scriptsize{± 0.99} & 66.46 \scriptsize{± 1.33} & 62.84 \scriptsize{± 1.08} \\
mistral & 50.17 \scriptsize{± 1.46} & 80.85 \scriptsize{± 0.81} & 83.49 \scriptsize{± 0.65} & 61.27 \scriptsize{± 0.49} & 75.59 \scriptsize{± 0.60} & 32.80 \scriptsize{± 2.10} & 80.79 \scriptsize{± 0.92} & 73.88 \scriptsize{± 1.23} & 67.35 \scriptsize{± 1.03} \\
\hline
\end{tabular}
\caption{Model performance (accuracy ± standard deviation) on various datasets.}
\label{tab:model_performance}
\end{table*}


\begin{table*}[ht]
\centering
\small
\begin{tabular}{l|cccccccc|c}
\hline
\textbf{Model} & \textbf{arc\_c} & \textbf{arc\_e} & \textbf{boolq} & \textbf{hellaswag} & \textbf{lambada} & \textbf{openbookqa} & \textbf{piqa} & \textbf{winogrande} & \textbf{avg} \\
\hline
mistral-7b-open-orca & 56.14 \scriptsize{± 1.45} & 79.59 \scriptsize{± 0.83} & 86.57 \scriptsize{± 0.60} & 81.73 \scriptsize{± 0.39} & 72.37 \scriptsize{± 0.62} & 45.60 \scriptsize{± 2.23} & 83.03 \scriptsize{± 0.88} & 73.24 \scriptsize{± 1.24} & 72.28 \scriptsize{± 1.03} \\
llama2-7b & 46.25 \scriptsize{± 1.46} & 74.58 \scriptsize{± 0.89} & 77.74 \scriptsize{± 0.73} & 75.99 \scriptsize{± 0.43} & 73.92 \scriptsize{± 0.61} & 44.20 \scriptsize{± 2.22} & 79.11 \scriptsize{± 0.95} & 69.14 \scriptsize{± 1.30} & 67.61 \scriptsize{± 1.07} \\
mistral-7b-capybara & 54.01 \scriptsize{± 1.46} & 78.54 \scriptsize{± 0.84} & 82.57 \scriptsize{± 0.66} & 78.74 \scriptsize{± 0.41} & 72.46 \scriptsize{± 0.62} & 44.80 \scriptsize{± 2.23} & 79.60 \scriptsize{± 0.94} & 71.03 \scriptsize{± 1.27} & 70.22 \scriptsize{± 1.05} \\
mistral-7b-open-hermes & 59.98 \scriptsize{± 1.43} & 81.65 \scriptsize{± 0.79} & 86.73 \scriptsize{± 0.59} & 81.77 \scriptsize{± 0.39} & 73.90 \scriptsize{± 0.61} & 44.20 \scriptsize{± 2.22} & 82.70 \scriptsize{± 0.88} & 73.56 \scriptsize{± 1.24} & 73.06 \scriptsize{± 1.02} \\
llama2-7b-nous-hermes & 49.74 \scriptsize{± 1.46} & 76.09 \scriptsize{± 0.88} & 80.00 \scriptsize{± 0.70} & 77.72 \scriptsize{± 0.42} & 72.99 \scriptsize{± 0.62} & 46.40 \scriptsize{± 2.23} & 79.76 \scriptsize{± 0.94} & 70.01 \scriptsize{± 1.29} & 69.09 \scriptsize{± 1.07} \\
llama2-7b-synth & 48.04 \scriptsize{± 1.46} & 76.77 \scriptsize{± 0.87} & 79.20 \scriptsize{± 0.71} & 76.04 \scriptsize{± 0.43} & 77.10 \scriptsize{± 0.59} & 43.40 \scriptsize{± 2.22} & 78.56 \scriptsize{± 0.96} & 69.30 \scriptsize{± 1.30} & 68.55 \scriptsize{± 1.07} \\
mistral-7b-synth & 59.39 \scriptsize{± 1.44} & 82.79 \scriptsize{± 0.77} & 86.15 \scriptsize{± 0.60} & 81.17 \scriptsize{± 0.39} & 78.36 \scriptsize{± 0.57} & 43.80 \scriptsize{± 2.22} & 82.37 \scriptsize{± 0.89} & 73.56 \scriptsize{± 1.24} & 73.45 \scriptsize{± 1.02} \\
llama2-7b-chat & 44.20 \scriptsize{± 1.45} & 69.74 \scriptsize{± 0.94} & 79.76 \scriptsize{± 0.70} & 75.50 \scriptsize{± 0.43} & 71.08 \scriptsize{± 0.63} & 43.80 \scriptsize{± 2.22} & 77.20 \scriptsize{± 0.98} & 66.46 \scriptsize{± 1.33} & 65.97 \scriptsize{± 1.09} \\
mistral-7b & 54.10 \scriptsize{± 1.46} & 79.50 \scriptsize{± 0.83} & 83.49 \scriptsize{± 0.65} & 81.12 \scriptsize{± 0.39} & 75.59 \scriptsize{± 0.60} & 44.40 \scriptsize{± 2.22} & 82.05 \scriptsize{± 0.90} & 73.88 \scriptsize{± 1.23} & 71.76 \scriptsize{± 1.03} \\
\hline
\end{tabular}
\caption{Model performance (accuracy ± standard deviation) on various datasets.}
\label{tab:model_performance_new}
\end{table*}




==> tables/ws.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table*}[h!]
\centering
\scriptsize
\begin{tabular}{l|cccccccc|c}
\hline
\textbf{Model} & \textbf{arc\_c} & \textbf{arc\_e} & \textbf{boolq} & \textbf{hellaswag} & \textbf{lambada} & \textbf{openbookqa} & \textbf{piqa} & \textbf{winogrande} & \textbf{average} \\
\hline 
\textsc{cb-match} & 57.40 \tiny{± 2.21} & 82.60 \tiny{± 1.70}  & 65.20 \tiny{± 2.13} & 72.00 \tiny{± 2.00} & 75.20 \tiny{± 1.93} & 43.80 \tiny{± 2.22} & 81.80 \tiny{± 1.73} & 74.60 \tiny{± 1.95} & 69.08 \\
\textsc{cb-ed} & 54.00 \tiny{± 2.23} & 79.60 \tiny{± 1.80} & 81.60 \tiny{± 1.73} & 71.20 \tiny{± 2.03} & 79.60 \tiny{± 1.80} & 44.60 \tiny{± 2.23} & 82.40 \tiny{± 1.70} & 73.20 \tiny{± 1.98} & 70.78 \\
\textsc{cb-mcqa} & 55.40 \tiny{± 2.22} & 80.20 \tiny{± 1.78} & 83.60 \tiny{± 1.66} & 71.80 \tiny{± 2.01} & 81.00 \tiny{± 1.76} & 44.40 \tiny{± 2.22} & 83.00 \tiny{± 1.68} & 74.60 \tiny{± 1.95} & 71.38 \\
\textsc{cb-select} & 55.60  \tiny{± 2.22} & 79.40 \tiny{± 1.81} & 82.60 \tiny{± 1.70} & 72.00 \tiny{± 2.00} & 80.60 \tiny{± 1.77} & 43.60 \tiny{± 2.22} & 82.60 \tiny{± 1.70} & 74.80 \tiny{± 1.94} & 71.40 \\
\hline
\textsc{cb-uni} & 58.70 \tiny{± 1.44} & 82.66 \tiny{± 0.78} & 79.97 \tiny{± 0.70} & 81.09 \tiny{± 0.39} & 78.46 \tiny{± 0.57} & 43.60 \tiny{± 2.22} & 81.77 \tiny{± 0.90} & 75.06 \tiny{± 1.22} & 72.66 \\
\textsc{cb-wsl} & 57.85 \tiny{± 1.44} & 82.37 \tiny{± 0.78} & 86.39 \tiny{± 0.60} & 81.36 \tiny{± 0.39} & 77.94 \tiny{± 0.58} & 44.60 \tiny{± 2.23} & 82.32 \tiny{± 0.89} & 74.19 \tiny{± 1.23} & 73.38\\
\textsc{cb-ws} & 57.76 \tiny{± 1.44} & 83.21 \tiny{± 0.77} & 85.23 \tiny{± 0.62} & 80.99 \tiny{± 0.39} & 78.23 \tiny{± 0.57} & 44.00 \tiny{± 2.22} & 82.32 \tiny{± 0.89} & 74.27 \tiny{± 1.23} & 73.25 \\
\end{tabular}
\caption{\textbf{WS performance analysis} ``CB*'' denotes our \alg tuned models on \mistral, where -\textsc{wsl} combines templates using downstream datasets with ground-truth outputs, -\textsc{ws} combines templates without ground-truth outputs and -\textsc{uni} is the uniform mixture. \textsc{match}, \textsc{ed}, \textsc{mcqa}, and \textsc{select}  are abbreviations for \match, \subj, \mcqa, \cqa individual \alg-tuned models.}
\label{tab:ws_perf}
\end{table*}


